Extracting Knowledge from Tools in LLM Agents

LLM agents commonly use knowledge-based tools and access their underlying files, databases, and search indexes through tool invocation. This integration improves agents' ability to provide domain-specific services but also introduces the risk of tool-mediated knowledge extraction: source content exposed to an agent for legitimate responses may be progressively recovered from its outputs, enabling reconstruction of the knowledge source behind a target tool. This paper systematically investigates this risk and identifies two challenges introduced by tool invocation: tool-selection uncertainty, where an agent may invoke a competing tool instead of the target tool, and tool-argument compression, where fine-grained query information may be lost when the agent generates tool arguments. To tackle these challenges, we propose ToolSiphon, a query-only extraction attack that introduces two complementary signals: a target-discriminative signal, implemented through Tool Contrastive Analysis, to steer queries toward the target tool; and a response-grounded factual signal, implemented through Evidence Chained Feedback, to mitigate argument compression and progressively expand extraction coverage. Across three types of knowledge-based tools and six domain-specific datasets, ToolSiphon recovers 74.3% of source records on average when coarse-grained information about non-target tools is available, with 83.2% textual recovery and 90.2% semantic similarity. Even without such information, it recovers 66.3% of source records. ToolSiphon also remains effective against representative defenses and on three real-world agent platforms.

==> sections/background.tex <==
\section{Background and Related Works}

\subsection{Knowledge-based Tools in Agent Platforms}
\label{Knowledge-based Tools}

Commercial agent-building platforms have become a common way to build and publish LLM agents. 
OpenAI reported that users created over three million custom GPTs within two months of the release of GPTs. 
Other major platforms, including Microsoft Copilot Studio, Salesforce Agentforce, Google Gemini Enterprise, and Dify, also provide interfaces for building agents, connecting data sources, adding actions or tools, and deploying them to users. 
A common pattern in these platforms is that developers connect agents to external knowledge sources to improve factuality, domain coverage, and task utility. 
We refer to such agent-accessible knowledge sources as \emph{knowledge-based tools}. 
In this section, we focus on the concrete forms of these tools.

Knowledge-based tools commonly appear in three forms. 
First, RAG tools retrieve top-\(k\) passages from a developer-provided corpus, such as manuals, policies, reports, or domain documents. 
Second, database tools expose structured records through SQL-like queries, filters, identifiers, or predefined API parameters. 
Third, search tools return top-\(k\) documents or snippets from web pages, enterprise documents, tickets, policies, or other indexed resources. 

However, this deployment pattern introduces a utility-security tradeoff. In traditional database security, fine-grained access control protects access-partitioned data through mechanisms such as role-based policies, row-level permissions, and document ACLs. Such controls remain important for knowledge-based tools that expose sensitive records or role-specific business data. Yet many tools in commercial agent platforms are connected for task-time knowledge support rather than direct data distribution. For instance, a tax-advisory agent may use filing manuals, public rulings, and expert guides to reason over tax questions. In these settings, knowledge that should not be exposed is better excluded from the shared tool than protected through assumed fine-grained authorization inside a general knowledge tool. 

Our measurements support this view: 56.2\% of 4,626 knowledge-based tools across three platforms (e.g., MCP Server) lacked explicit access control, as did 74.9\% of 735 tools in Dify’s official plugin ecosystem. Thus, when fine-grained access control is not the default security foundation, KTE captures a malicious behavior in which seemingly ordinary task-oriented interactions can be exploited to reconstruct the knowledge supplied by such tools.

\subsection{Tool Invocation in Agent}

Unlike traditional knowledge sources that expose a direct query interface, knowledge-based tools are accessed through tool invocation. 
A tool is exposed to the Core LLM through a standardized interface, typically consisting of a name, a natural-language description, and a parameter schema. 
Tool invocation consists of two steps: \emph{tool selection} and \emph{parameter synthesis}. 
In tool selection, the model compares the user request and conversation context with available tool descriptions to decide whether a tool is needed and which tool to invoke. 
This process is semantic rather than exact, since it depends on how the model interprets both the request and the tool descriptions. 
In parameter synthesis, the model converts the natural-language request into structured inputs required by the selected tool, such as a search query and a top-\(k\) value. 
This step may extract entities, rewrite the request, compress multi-part intents, or infer missing fields to fit the tool schema.

Formally, let each tool be represented as
\(
T_i = \langle n_i, d_i, P_i \rangle,
\)
where \(n_i\), \(d_i\), and \(P_i\) denote the tool name, description, and parameter schema. 
Given a query \(q\), the agent selects a tool and synthesizes its parameters:
\begin{equation}
    T^\ast = \mathrm{Select}(q, \{T_1,\ldots,T_N\}), 
\theta^\ast = \mathrm{Param}(q, T^\ast).
\end{equation}

The resulting invocation \((T^\ast,\theta^\ast)\) returns content that is incorporated into the agent's subsequent reasoning, which may include additional tool invocations, before the final response:
\begin{equation}
\label{tool_invocarion_path}
    q \rightarrow \text{Core LLM} \rightarrow (T^\ast,\theta^\ast) \rightarrow ... \rightarrow \text{Response}.
\end{equation}

For example, a legal case search tool may be exposed as


\begin{tcolorbox}[
    colback=gray!3,
    colframe=black!60,
    title=\texttt{Example 1. legal\_case\_search\_Tool},
    fonttitle=\bfseries\ttfamily,
    sharp corners,
    boxrule=0.6pt,
    left=8pt,
    right=8pt,
    top=6pt,
    bottom=6pt
]
\textbf{Description.} Search legal cases relevant to a company, statute, or legal issue.

\textbf{Parameters.}
\[
\begin{array}{ll}
\texttt{query} & \text{Legal issues or company description.} \\
\texttt{top\_k} & \text{Number of most relevant cases to retrieve.}
\end{array}
\]
\end{tcolorbox}

For a request about prior cases involving a company, the Core LLM may synthesize
\begin{tcolorbox}[
    colback=gray!3,
    colframe=black!60,
    title=\texttt{Example 2.} legal\_case\_search Parameter Synthesis,
    fonttitle=\bfseries,
    sharp corners,
    boxrule=0.5pt,
    left=7pt,
    right=7pt,
    top=3pt,
    bottom=3pt,
    before skip=4pt,
    after skip=4pt
]
\small
\centering
\(\theta^\ast =
\{\texttt{query}=\texttt{``Acme Tax Dispute'’},\, \texttt{top\_k}=5\}\).
\end{tcolorbox}
Thus, the user does not directly query the underlying knowledge source; the request is first routed through tool selection and parameter synthesis.

\subsection{Related Work}

Prior work relevant to KTE falls into three categories: black-box attacks on LLMs and agents, extraction attacks against RAG or memory, and tool-centric attacks on agent systems.


\mypara{Black-box attacks on LLMs and agents.}
Prompt injection, jailbreaking, and denial-of-service attacks study how adversarial or perturbed inputs induce undesired model behavior, such as following untrusted instructions, producing prohibited content, or consuming excessive computation. 
Their perturbations may sometimes affect tool selection, but their objectives are typically single-shot behavioral failures rather than sustained reconstruction of tool-supplied knowledge. 
In KTE, the attacker must iteratively expand ordinary task-oriented interactions while observing only indirect feedback through the agent's final responses, making it difficult to infer whether a target tool was invoked or whether the content came from the intended source.


\mypara{Extraction from RAG and memory.}
A second line of work studies extraction from RAG systems or agent memory. 
These settings are often closer to a direct extraction path,
\(
\text{query} \rightarrow \text{RAG / memory} \rightarrow \text{LLM response},
\)
where output feedback can guide query mutation and corpus traversal. 
In KTE, however, the query must pass through the agent's tool-invocation process before reaching a knowledge-based tool. 
Tool selection may route the query to a related but non-target tool, while parameter synthesis may rewrite or compress semantic cues into tool-specific inputs. 
As a result, methods designed for direct RAG or memory extraction may be less effective in KTE, because their feedback signals are filtered through tool selection and parameter synthesis.

\mypara{Tool-misuse attacks on agents.}
Recent work also studies attacks that manipulate agent tool selection. 
A common setting assumes a malicious tool developer who modifies tool names, descriptions, or metadata to influence the agent's tool-selection process. 
This differs from KTE, where the attacker is an ordinary user of a deployed agent and cannot alter tool definitions. 
Such work shows that tool interfaces are an important attack surface, but it does not address user-originated knowledge reconstruction through normal tool invocations

As shown in \autoref{tool_invocarion_path}, KTE studies knowledge extraction through the agent-mediated tool-invocation process rather than through direct access to a RAG endpoint, memory module, or tool metadata. 
It therefore complements prior work by focusing on whether ordinary task-oriented interactions can be expanded into unintended reconstruction of knowledge supplied by tools.

==> sections/challenge.tex <==
\subsection{Tool Invocation in Agent}
\label{tool invocation}

Unlike traditional knowledge sources that expose a direct query interface, knowledge-based tools are accessed through tool invocation \cite{schick2023toolformer,chen2024t,qin2024toolllm}. Tool invocation has two steps: \emph{tool selection} and \emph{parameter synthesis} \cite{qin2024toolllm,patil2024gorilla}. In tool selection, the agent's core LLM uses the user query, current context, and available tool descriptions to decide whether to invoke a tool and which tool to invoke \cite{schick2023toolformer,chen2024t}. In parameter synthesis, the core LLM converts the natural-language query into parameters that match the selected tool's schema. This process may extract entities, rewrite the query, compress multi-part intent, or infer missing fields \cite{schick2023toolformer,chen2024t,qin2024toolllm}.

Formally, given a user query \(q\), context \(c_t\), and available tools \(\mathcal{T}=\{T_1,\ldots,T_N\}\), the core LLM makes a step-wise tool-selection decision:
\(
    T_t^{sel}
    =
    \mathrm{Select}(q,c_t,\mathcal{T})
    \in \mathcal{T}\cup\{\bot\},
\)
where \(\bot\) denotes no tool invocation. 
If \(T_t^{sel}=\bot\), the agent stops invoking tools and produces the final response. 
Otherwise, for the selected tool \(T_t^{sel}=\langle n_t,d_t,P_t\rangle\), it synthesizes a concrete parameter assignment:
\(
    \theta_t^{\ast}
    =
    \mathrm{Param}(q,c_t,T_t^{sel}),
    \theta_t^{\ast} \models P_t .
\)
The tool executes its internal function over the corresponding knowledge source:
\(
    y_t = F_{T_t^{sel}}(\theta_t^{\ast};\mathcal{K}_{T_t^{sel}}).
\)
The returned content \(y_t\) is incorporated into the agent context, yielding \(c_{t+1}\). 
The agent may then repeat the same process until it selects \(\bot\):
\begin{equation}
\label{eq:agent_invocation_path}
        q \rightarrow
    \bigl[(T_i^{sel},\theta_i^{\ast},y_i)\rightarrow c_{i+1}\bigr]_{i=1}^{m}
    \rightarrow \mathrm{Response}.
\end{equation}

For example, suppose an agent has access to a legal case search tool \(T_{case}\) and a statute search tool \(T_{statute}\). For a user query such as ``find prior cases involving Acme's tax dispute,'' the agent may perform multiple tool-invocation steps:

\begin{tcolorbox}[
    colback=gray!3,
    colframe=black!60,
    title=\texttt{Example 3: Tool Invocation},
    fonttitle=\bfseries\ttfamily,
    sharp corners,
    boxrule=0.6pt,
    left=8pt,
    right=8pt,
    top=6pt,
    bottom=6pt
]
\textbf{Step 1: }
\(
T_1^{sel}=T_{\mathrm{case}}
\),
\(
\theta_1^{\ast}
=
\{\texttt{query}=\text{``Acme tax dispute''},\;
  \texttt{top\_k}=5\}
\)

\textbf{Step 2:} 
\(
T_2^{sel}=T_{\mathrm{statute}}
\),
\(
\theta_2^{\ast}
=
\{\texttt{query}=\text{``tax dispute''},\;
  \texttt{juris}=\text{``federal''}\}
\)

\textbf{Final Answer.}
\(
T_3^{sel}=\bot\rightarrow
\)
Final Answer
\end{tcolorbox}



\mypara{Empirical Validation.}
We conduct two exploratory experiments to examine the impact of tool invocation on existing extraction attacks. 
The first measures how tool selection affects extraction fidelity, since selecting related non-target tools may mix target knowledge with irrelevant or weakly related content. 
The second measures how parameter synthesis affects extraction coverage, since rewritten or compressed parameters may not reach portions of the target knowledge source.

These experiments are diagnostic rather than end-to-end evaluations of knowledge-source reconstruction.
Specifically, following prior extraction studies \cite{jiang2024rag,qi2024follow,wang2025silent,wang2025unveiling}, we use two metrics to characterize these exploratory results, instead of using the overall KSR metric. 
(1) SS reflects how faithfully extracted outputs match the target source, while (2) EC reflects how much of the target source is recovered. The detailed definitions of SS and EC are provided in \autoref{sec:setup}.

\textit{I. For Tool Selection.} 
To isolate how tool selection affects KTE stress testing, we compare extraction under different tool environments. We first distinguish tools by the user intents they support, where an intent refers to the task type or information need a tool is designed to serve, such as answering symptom questions, retrieving refund policies, or searching product manuals. For a target knowledge-based tool \(T^\star\), we call another tool \(T_j\) a \emph{related tool} if it supports overlapping user intents with \(T^\star\) but uses a different knowledge source or parameter schema. We call \(T_j\) an \emph{unrelated tool} if its supported intents do not overlap with those of \(T^\star\).

\begin{tcolorbox}[
    colback=gray!3,
    colframe=black!60,
    title=\texttt{Example 4: Related Tools},
    fonttitle=\bfseries\ttfamily,
    sharp corners,
    boxrule=0.6pt,
    left=8pt,
    right=8pt,
    top=6pt,
    bottom=6pt
]
\textbf{Target tool.}
\(T^\star\): a HealthCareMagic QA retriever backed by doctor-patient consultation records.

\textbf{Related tool.}
\(T_j\): a medical guideline retriever backed by clinical guideline documents.

\textbf{Shared intent.}
Both tools may be selected for questions about symptoms, diagnosis, or treatment.
\end{tcolorbox}

We adapt RAG-Thief, IKEA, and MEXTRA to a HealthcareMagic-based target tool and evaluate them under four tool environments: target-only, target with related tools, target with unrelated tools, and a mixed setting. As shown in \autoref{fig:overall_comparison}, related tools substantially reduce extraction fidelity. For example, IKEA's SS drops by \(0.29\) when related tools are added and by more than \(0.33\) in the mixed setting, whereas adding unrelated tools causes only a \(0.03\) drop.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{fig/rag-method-scenario-ss-optimized.pdf}
    \caption{Impact of tool selection for baseline attacks.}
    \label{fig:overall_comparison}
\end{figure}

\textit{II. For parameter synthesis}, to isolate parameter synthesis, we use a single target tool and evaluate the same methods across RAG-based, database-backed, and search-tool implementations. We compare their original extraction settings, where the generated queries act more directly on the target knowledge source, with the KTE setting, where the agent must first convert those queries into tool parameters. As summarized in \autoref{tab:C2_results}, all methods achieve higher EC in their original settings but degrade after agent-mediated parameter synthesis. Even for RAG-based tools, EC drops by \(0.27\) on average; for database-backed tools, where exact predicates are required, the drop exceeds \(0.45\).

\begin{table}[th]
\centering
\caption{Impact of parameter synthesis on EC.}
\label{tab:C2_results}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccc}
\toprule
 & Origin & RAG & Database & Search \\
\midrule
RAG-Thief & 0.672 & 0.415\,(0.257$\downarrow$) & 0.238\,(0.434$\downarrow$) & 0.294\,(0.378$\downarrow$) \\
IKEA      & 0.743 & 0.443\,(0.300$\downarrow$) & 0.272\,(0.471$\downarrow$) & 0.350\,(0.393$\downarrow$) \\
MEXTRA    & 0.727 & 0.474\,(0.253$\downarrow$) & 0.276\,(0.451$\downarrow$) & 0.361\,(0.366$\downarrow$) \\
\bottomrule
\end{tabular*}
\end{table}

==> sections/problem.tex <==
\section{Problem Statement}

\subsection{KTE Problem Formulation}
\label{Formulation}

We define knowledge-tool extraction (KTE) as a black-box data extraction attack against an agent equipped with a private knowledge tool. Let \(\mathcal{A}\) denote the deployed agent, and let \(D=\{r_1,\ldots,r_N\}\) denote the private knowledge source accessed by the tool, where each \(r_i\) is a source-level record such as a rule, example, template, case, or knowledge chunk. The adversary has no direct access to \(D\), but can interact with \(\mathcal{A}\) through its public interface.

KTE is not defined by whether a response contains private knowledge, since legitimate tool use may also expose task-relevant fragments of the private source. Instead, KTE is defined by the adversary's attempt to turn repeated interactions with the agent into a reusable reconstruction of the underlying knowledge source. The adversary issues adaptive queries \(q_1,\ldots,q_T\), observes responses \(y_1,\ldots,y_T\), and constructs an extracted dataset \(\hat{D}=\{\hat{r}_1,\ldots,\hat{r}_M\}\).

A harmful KTE attack should satisfy two conditions. First, it should achieve broad coverage of the private knowledge source, rather than recovering only isolated facts. Second, it should preserve the fidelity of recovered records: extracted records should correspond to genuine source records, retain their semantic and field-level content, and avoid excessive duplication, irrelevant content, or hallucinated entries. We refer to the overall degree to which \(\hat{D}\) reconstructs \(D\) under these conditions as the knowledge-source reconstruction score \(KSR(D,\hat{D})\). Higher KSR indicates greater KTE risk because the extracted dataset more closely approximates the private knowledge source. Section~5.2 specifies how KSR is operationalized in our evaluation.

% We formalize knowledge-tool extraction (KTE) as a black-box data extraction attack against an agent equipped with a private knowledge tool. Let \(\mathcal{A}\) denote the agent, and let \(D=\{r_1,\ldots,r_N\}\) denote the private knowledge source accessed by the tool. Each \(r_i\) is a source-level record, such as a rule, example, template, case, or knowledge chunk. The adversary cannot directly access \(D\), but can interact with \(\mathcal{A}\) through its public interface.

% This distinction separates KTE, which extracts and reconstructs the underlying knowledge source, from legitimate use, which applies tool-provided knowledge to a bounded task. We therefore define extraction not by a single response containing private knowledge, but by an interaction sequence that recovers source-level records and organizes them into a reusable dataset.

% In a KTE attack, the adversary issues adaptive queries \(q_1,\ldots,q_T\) and observes responses \(y_1,\ldots,y_T\). From these interactions, the adversary constructs an extracted dataset
% \(
% \hat{D}=\{\hat{r}_1,\ldots,\hat{r}_M\}.
% \)
% The goal of KTE is to reconstruct the underlying knowledge source \(D\), rather than elicit isolated facts. A successful extraction should cover many target records, preserve their semantic and field-level content, and avoid duplicated, irrelevant, or hallucinated outputs.

% For each source record \(r_i\) and extracted record \(\hat{r}_j\), we compute two similarity scores. First, we compute a semantic similarity score \(S_{ij}\) using a semantic encoder \(E(\cdot)\) (e.g., text-embedding-3-small).
% Second, we compute a field-level content similarity score \(F_{ij}\) using ROUGE-L F1. 

% We combine semantic similarity and field-level content similarity into a record-level reconstruction score:
% \(
% Q_{ij}=\sqrt{S_{ij}F_{ij}}.
% \)
% We use the geometric mean because a high reconstruction score should require both semantic equivalence and content-level recovery.

% To avoid counting duplicated outputs multiple times, we compute a maximum-weight one-to-one matching between source records and extracted records:
% \begin{equation}
%     \mathcal{M}^{*}
% =
% \arg\max_{\mathcal{M}}
% \sum_{(i,j)\in\mathcal{M}} Q_{ij},
% \end{equation}
% where each \(r_i\in D\) and each \(\hat{r}_j\in\hat{D}\) can appear in at most one matched pair. The quality-adjusted amount of reconstructed source content is
% \(
% C=\sum_{(i,j)\in\mathcal{M}^{*}} Q_{ij}.
% \)

% We define the quality-adjusted reconstruction recall as
% \(
% R_{\mathrm{rec}}=\frac{C}{N},
% \)
% which measures the fraction of the private knowledge source reconstructed after accounting for partial errors and duplicated outputs. We also define extraction precision as
% \(
% P_{\mathrm{ext}}=\frac{C}{M},
% \)
% which measures how much of the extracted dataset corresponds to valid source content. Finally, we summarize reconstruction quality using
% \begin{equation}
%     KSR=
% \frac{2\cdot R_{\mathrm{rec}}\cdot P_{\mathrm{ext}}}
% {R_{\mathrm{rec}}+P_{\mathrm{ext}}},
% \end{equation}
% and set \(KSR=0\) when \(R_{\mathrm{rec}}+P_{\mathrm{ext}}=0\). 

% Under this formulation, the objective of a KTE attack is
% \(
%     \max_{\hat{D}} \; KSR(D,\hat{D}),
% \)
% subject to the constraint that \(\hat{D}\) is constructed only from black-box interactions with \(\mathcal{A}\).

\subsection{Threat Model}

\mypara{Target System.} We consider a deployed agent \(A\) equipped with multiple knowledge-based tools
\(\mathcal{T}_A=\{T_1,\ldots,T_N\}\), where each tool \(T_i\) exposes an underlying knowledge source \(D_i\).
In our setting, the target tool \(T_t\in\mathcal{T}_A\) is accompanied by related tools
\(\mathcal{R}_A(T_t)\subseteq\mathcal{T}_A\setminus\{T_t\}\), which may serve the same user request as \(T_t\) but return knowledge from different sources or evidence types.
This is a practical configuration: for example, AutoGen's official literature-review example configures both an Arxiv search component and a Google search component for the same high-level task of finding papers related to a given topic, while the two components retrieve evidence from different sources.
The presence of related tools represents a harder KTE scenario because it increases the possibility that a request intended for \(T_t\) is selected for a related non-target tool before parameter synthesis.
This paper focuses on this more challenging setting.

\mypara{Attacker's Goal.} Given a deployed agent \(A\) with a set of knowledge-based tools \(\mathcal{T}_A\), the attacker targets a specific knowledge-based tool \(T_t\in\mathcal{T}_A\) and aims to reconstruct its internal knowledge source \(D_t\) through ordinary interactions with the agent.
Given a query budget \(B\), the attacker adaptively submits a sequence of task-oriented requests
\(
Q_B=(q_1,\ldots,q_B)
\)
and observes only the agent's final responses
\(
R_B=(r_1,\ldots,r_B).
\)
From these responses, the attacker constructs an extracted knowledge set \(\widehat{D}_t\).
We use KSR, introduced in \autoref{Formulation}, to measure the fraction of the target internal knowledge source recovered by \(\widehat{D}_t\).
The attacker's objective is to maximize KSR under the query budget:
\(
    \max_{Q_B:\ |Q_B|\le B} \ \mathrm{KSR}(\widehat{D}_t,D_t).
\)


\mypara{Attacker knowledge.}
We assume a black-box attacker who has no access to the agent's system prompt, model weights, execution traces, tool-selection decisions, synthesized parameters, raw tool outputs, or backend knowledge sources.
The attacker only knows the commercial agent's public-facing functional information, such as its name, description, task category, advertised capability, and example queries.
This information is a necessary part of commercial agent deployment, since agents must communicate their intended use to attract users for specific tasks.

We consider two adversaries that differ only in their knowledge of tool metadata.
For \underline{\textit{Adversary 1 (A1)}}, the attacker is assumed to observe user-facing tool metadata, such as capability descriptions or source labels, but not internal parameter schemas.
For example, Scholar GPT publicly advertises scholarly source labels such as Google Scholar, PubMed, and arXiv.
For \underline{\textit{Adversary 2 (A2)}}, the attacker is assumed to be unaware of exact tool metadata, including internal tool names, descriptions, schemas, and related-tool metadata.
However, the attacker knows the public scenario of the commercial agent and the general nature of the target tool \(T_t\)'s knowledge function.
For example, Consensus is publicly positioned as a research assistant for academic papers, indicating that a target tool in this agent may provide scientific literature retrieval.
Without such coarse knowledge of \(T_t\), targeted KTE would reduce to untargeted exploration rather than reconstruction of a specific internal knowledge source \(D_t\).

\mypara{Attacker capabilities.}
An attack is stronger if it requires fewer attacker capabilities.
We consider a constrained black-box attacker who can only submit ordinary task-oriented requests and observe final responses.
The attacker cannot modify prompts, tools, knowledge sources, or workflows, directly invoke backend tools, or inspect intermediate results.
The attacker may use an LLM to generate follow-up requests.
In A2, where exact related-tool metadata is hidden, the attacker may synthesize \emph{shadow related tools}: proxy descriptions of plausible related tools generated from the agent's public-facing function and the coarse function of \(T_t\).
They are used to approximate non-target tools that may compete with \(T_t\) during tool selection and to identify functionality that better distinguishes \(T_t\), without accessing actual tool metadata or backend knowledge sources.

\mypara{Out of scope.}
As shown in \autoref{Knowledge-based Tools}, fine-grained authorization at the knowledge-based tool level is not universal in current commercial agent ecosystems.
We do not study tools protected by explicit fine-grained access control.
Instead, we focus on KTE risks for tools without such permissions, which account for a substantial fraction of the tools observed in \autoref{Knowledge-based Tools}.

==> sections/related.tex <==
\section{Related Work}


\mypara{Prompt injection attacks.}
Prompt injection attacks manipulate LLM-integrated applications by placing malicious instructions in user inputs or external content later consumed by the model. For a complete file or webpage returned to the agent, such instructions may cause the agent to reveal the retrieved content. However, knowledge-based tools often return only a small number of records per call, and the user query must first be converted into a tool invocation. Prompt injection therefore does not directly provide the continuous, coverage-oriented extraction capability needed to reconstruct an entire tool-backed knowledge source.


\mypara{Data extraction from RAG and memory.}
Recent work studies black-box extraction from RAG systems and agent memory. RAG-Thief shows that attackers can recover private knowledge from retrieval-augmented systems through adaptive querying. IKEA further improves RAG extraction by using benign-looking anchored queries to explore the knowledge base. MEXTRA studies extraction from agent memory, showing that private memory contents can be recovered from deployed agents through black-box interactions. These works demonstrate that external knowledge and memory can leak through model responses. Our setting differs in the extraction path. Existing RAG and memory attacks typically follow a direct path, query $\rightarrow$ retriever/memory $\rightarrow$ LLM response. In KTE, the path is query $\rightarrow$ tool selection $\rightarrow$ parameter synthesis $\rightarrow$ target tool $\rightarrow$ LLM response. This intermediate tool-invocation layer can redirect queries to related tools or rewrite their parameters, making existing extraction methods less effective.

\mypara{Defense.}
Existing defenses include general safeguards, such as keyword filtering, intent detection, and system-prompt constraints, which block suspicious requests or instruct agents not to disclose protected content. Specialized defenses protect the knowledge pipeline more directly: SAGE replaces private records with synthetic data, DP-based RAG limits the influence of individual records, and RAGFort modifies retrieval and generation to reduce knowledge reconstruction.
However, these defenses were not designed for extraction accumulated through repeated tool calls mediated by tool selection and parameter synthesis.
